a Decision-Tree based Moment-of-Fluid (DTMOF) Method in 3D rectangular hexahedrons

The moment-of-fluid (MOF) method is an extension of the volume-of-fluid method with piecewise linear interface construction (VOF-PLIC). By minimizing the least square error of the centroid of the cutting polyhedron, the MOF method reconstructs the linear interface without using any neighboring information. Traditional MOF involves iteration while finding the optimized linear reconstruction. Here, we propose an alternative approach based on a machine learning algorithm: Decision Tree algorithm. A training data set is generated from a list of random cuts of a unit cube by plane. The Decision Tree algorithm extracts the input-output relationship from the training data, so that the resulting function determines the normal vector of the reconstruction plane directly, without any iteration. The present method is tested on a range of popular interface advection test problems. Numerical results show that our approach is much faster than the iteration-based MOF method while provides compatible accuracy with the conventional MOF method.

==> figures.tex <==
%<*fig:sketchmof>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.3\textwidth]{sketch_mof_centroid.pdf}
    \caption{2D view of the MOF reconstruction. The red line is the true interface and the blue dashed line is the reconstructed interface by MOF. The centroid of the reconstruct red interface (blue cross) is the optimized centroid that minimized the distance between the reconstructed centroid and the referencehttps://www.overleaf.com/project/5f7a88e90eac1a00019593c8 centroid (red cross) with same volume fraction.
    }
    \label{fig:sketchmof}
\end{figure}
%</fig:sketchmof>

%<*fig:dt>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{tree.pdf}
    \caption{
    Representative tree structure from the training data set in section 3  (All float numbers are represented with 2 significant digits). The data set is divided into two data sets recursively with a threshold value based on one of the input features. Branches to the left (right) represent the division of data points less equal (greater than) the threshold value.  The values of the output variables in the output nodes are mean values of the data in the corresponding partition. Note that the Decision Tree does not have to be a full binary tree, the output nodes (leaf nodes) may not always be located at the same level.
    }
    \label{fig:dt}
\end{figure}
%</fig:dt>


%<*fig:xyzptf>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{volume.pdf}
    \caption{(a) Locus of centroids for volume fraction $C$ in the region of  $\Omega_1(x,y,z) = [-0.5,0.5] \times [-0.5,0.5] \times [-0.5,0.5]$  and (b) corresponding locus of centroids in the region of  $\Omega_2(\phi,\theta,C)=[-\pi,\pi] \times [0,\pi] \times [0,1]$ }
    \label{fig:xyzptf}
\end{figure}
%</fig:xyzptf>

%<*fig:dperror>
\begin{figure}[htbp]
    \centering
    \subfigure[training data-set]{\includegraphics[width=0.5\textwidth]{dp1.png}} 
    \subfigure[test data-set]{\includegraphics[width=0.5\textwidth]{dp3.png}} 
    \caption{
    The value of $\Delta \phi$ in the region of  $\Omega_2(\phi,\theta,C)=[-\pi,\pi] \times [0,\pi] \times [0,1]$,
    for (a) training data-set (b) test data-set}
    
    \label{fig:dperror}
\end{figure}
%</fig:dperror>

%<*fig:dterror>
\begin{figure}[htbp]
    \centering
    \subfigure[training data-set]{\includegraphics[width=0.5\textwidth]{dt1.png}}
    \subfigure[test data-set]{\includegraphics[width=0.5\textwidth]{dt3.png}}
    \caption{
    The value of $\Delta \theta$ in the region of  $\Omega_2(\phi,\theta,C)=[-\pi,\pi] \times [0,\pi] \times [0,1]$,
    for (a) training data-set (b) test data-set
    }
    \label{fig:dterror}
\end{figure}
%</fig:dterror>


% %<*fig:trainingerror>
% \begin{figure}[htbp]
%     \centering
%     \subfigure[]{\includegraphics[width=0.5\textwidth]{figures/mof3dplot/dt3.png}}
%     \subfigure[]{\includegraphics[width=0.5\textwidth]{figures/mof3dplot/dp3.png}}
%     \caption{(a) Locus of centroids for volume fraction $C$ in the region of 
%     $\Omega_1(x,y,z) = [-0.5,0.5] \times [-0.5,0.5] \times [-0.5,0.5]$ 
%     and (b) corresponding locus of centroids in the region of 
%     $\Omega_2(\phi,\theta,C)=[-\pi,\pi] \times [0,\pi] \times [0,1]$
%     }
%     \label{fig:trainingerror}
% \end{figure}
%</fig:trainingerror>


%<*fig:DTConvergence>
\begin{figure}[htbp]
    \centering
    \subfigure[]{\includegraphics[height=0.3\textwidth]{node_time.pdf}}
    \subfigure[]{\includegraphics[height=0.3\textwidth]{error.pdf}}
    \caption{Error, cpu time and total leaf count with the change of the tree depth.
    }
    \label{fig:DTconvergence}
\end{figure}
%</fig:DTConvergence>

%<*fig:translationinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{sketch1.pdf}
    \caption{Initial setup of translation tests.
    }
    \label{fig:translationinit}
\end{figure}
%</fig:translationinit>

%<*fig:translationresult2d>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{translation_slice.pdf}
    \caption{Comparison of 2D slice of $x-y$ plance at $z=0.15$ for the translation problem at $t=T$.
    }
    \label{fig:translationresult2d}
\end{figure}
%</fig:translationresult2d>

%<*fig:translationresult3d>
\begin{figure}[htbp]
    \centering
    \subfigure[Exact]
    {\includegraphics[width=0.4\textwidth]{exact1.png}}
    \subfigure[ELVIRA]
    {\includegraphics[width=0.4\textwidth]{elvira1.png}} \\

    \subfigure[Iteration-based MOF]
    {\includegraphics[width=0.4\textwidth]{mof1.png}}
    \subfigure[DTMOF]
    {\includegraphics[width=0.4\textwidth]{dtmof1.png}}
    \caption{Comparison of the material interface of the translation problem at $t=T$ with grid resolution of $100\times 100 \times 50$.
    }
    \label{fig:translationresult3d}
\end{figure}
%</fig:translationresult3d>

%<*fig:zalesakinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{sketch2.pdf}
    \caption{Initial setup and parameters of Zalesak's rotation test
    }
    \label{fig:zalesakinit}
\end{figure}
%</fig:zalesakinit>

%<*fig:zalesakresult2d>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{zalesak_slice.pdf}
    \caption{Comparison of 2D slice of $x-y$ plance at $z=0.15$ for the Zalesak's problem at $t=T$.
    }
    \label{fig:zalesakresult2d}
\end{figure}
%</fig:zalesakresult2d>

%<*fig:zalesakresult3d>
\begin{figure}[htbp]
    \centering
    \subfigure[ELVIRA]
    {\includegraphics[width=0.3\textwidth]{elvira2.png}}
    \subfigure[Iteration-based MOF]
    {\includegraphics[width=0.3\textwidth]{mof2.png}}
    \subfigure[DTMOF]
    {\includegraphics[width=0.3\textwidth]{dtmof2.png}} \\
    \caption{Comparison of material interface of the Zalesak's problem at $t=T$ with grid resolution of $100\times 100 \times 50$.
    }
    \label{fig:zalesakresult3d}
\end{figure}
%</fig:zalesakresult3d>

%<*fig:reversevortexinit>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{sketch3.pdf}
    \caption{The initial setup and parameters for reverse vortex case (deformation test)
    }
    \label{fig:rvinit}
\end{figure}
%</fig:reversevortexinit>


%<*fig:reversevortexevolution>
\begin{figure}[htbp]
    \centering
    \subfigure[$t=0$]
    {\includegraphics[width=0.3\textwidth]{0.png}}
    \subfigure[$t=1/8 T$]
    {\includegraphics[width=0.3\textwidth]{375.png}} 
    \subfigure[$t=1/4 T$]
    {\includegraphics[width=0.3\textwidth]{750.png}} \\

    \subfigure[$t=3/8 T$]
    {\includegraphics[width=0.3\textwidth]{1125.png}}
    \subfigure[$t=1/2 T$]
    {\includegraphics[width=0.3\textwidth]{1500.png}} 
    \subfigure[$t=5/8 T$]
    {\includegraphics[width=0.3\textwidth]{1875.png}} \\

    \subfigure[$t=3/4 T$]
    {\includegraphics[width=0.3\textwidth]{2250.png}}
    \subfigure[$t=7/8 T$]
    {\includegraphics[width=0.3\textwidth]{2625.png}} 
    \subfigure[$t= T$]
    {\includegraphics[width=0.3\textwidth]{3000.png}} \\
    \caption{Evolution of the reverse vortex computed from DTMOF method with grid resolution of $200 \times 200 \times 200$}
    \label{fig:reversevortexevolution}
\end{figure}
%</fig:reversevortexevolution>

%<*fig:reversevortex100result>
\begin{figure}[htbp]
    \centering
    \subfigure[$t=1/2 T$ (ELVIRA)]
    {\includegraphics[width=0.3\textwidth]{elvira31.png}}
    \subfigure[$t=1/2 T$ (Iteration-based MOF)]
    {\includegraphics[width=0.3\textwidth]{mof31.png}} 
    \subfigure[$t=1/2 T$ (DTMOF)]
    {\includegraphics[width=0.3\textwidth]{dtmof31.png}} \\
    \subfigure[$t=T$ (ELVIRA)]
    {\includegraphics[width=0.3\textwidth]{elvira32.png}}
    \subfigure[$t=T$ (Iteration-based MOF)]
    {\includegraphics[width=0.3\textwidth]{mof32.png}} 
    \subfigure[$t=T$ (DTMOF)]
    {\includegraphics[width=0.3\textwidth]{dtmof32.png}} \\

    \caption{Comparison of the material interface of the reverse vortex problem at $t=1/2 T$ and $t=T$ with grid resolution of $100\times 100 \times 100$}
    \label{fig:reversevortex100result}
\end{figure}
%</fig:reversevortex100result>

%<*fig:reversevortexresult2d>
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{vortex_slice.pdf}
    \caption{Comparison of the 2D slice of the reverse vortex problem at $t=T$}
    \label{fig:reversevortexresult2d}
\end{figure}
%</fig:reversevortexresult2d>

==> tables.tex <==
%<*tab:mlstatic>
\begin{table}[tbhp]
  \centering
  \caption{The centroid error and run-time ratio from different methods on test data-set}
  \label{tab:mlstatic}
\begin{tabular}{@{}llll@{}}
\toprule
Method                                       & $E_c$ & $R^2$ & Run-time ratio \\ 
\midrule
Decision Tree (Current method)          & $3.28 \times 10^{-3}$     &  0.977  &  1    \\
Random Forest  (10 estimators)      & $2.40 \times 10^{-3}$     &  0.981  &  11.62     \\
Random Forest  (100 estimaters)     &  $2.24 \times 10^{-3}$    &  0.982  &  164.04     \\
Nueral Network (Hidden layer sizes: (20,15,10,5))  &  $8.14 \times 10^{-3}$    &  0.732  &   3.51    \\
Nueral Network (Hidden layer sizes: (100,100))         &  $3.21 \times 10^{-3}$    &  0.971  &   11.88    \\
Analytic MOF \citep{milcent_moment--fluid_2020}                                          &  $1.69 \times 10^{-9} $    &      1.000          &  18.77     \\
Conventional MOF \citep{dyadechko_moment--fluid_2005}                                       & $1.69 \times 10^{-9}$   &      1.000          &  2966.67     \\ \bottomrule
\end{tabular}
\end{table}
%</tab:mlstatic>

%<*tab:translationerror>
\begin{table}[tbhp]
  \centering
  \caption{Geometrical error and run-time ratio in translation test}
  \label{tab:translationerror}
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{$E_r$}                                                                                               &  \multicolumn{1}{c}{\multirow{2}{*}{Run-time ratio}} \\ \cmidrule(lr){2-5}
\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{Cube} & \multicolumn{1}{c}{sphere} & \multicolumn{1}{c}{Tilt cube} & \multicolumn{1}{c}{letter A} & \multicolumn{1}{c}{}                      \\ \midrule
Grid: $50 \times 50 \times 25$                                          &                          &                            &                               &                              &                                    \\ \midrule
ELVIRA \citep{pilliod_second-order_2004}                                      & 1.14e-1                 & 1.46e-1                   & 2.38e-1                      & 2.48e-1                      & 79.2                                      \\
Analytic MOF \citep{milcent_moment--fluid_2020}                               & 4.23e-2                 & 2.63e-2                   & 8.74e-2                      & 7.28e-2                       & 7.71                                      \\
Conventional MOF \citep{dyadechko_moment--fluid_2005}                                & 4.21e-2                 & 2.63e-2                   & 8.74e-2                      & 7.28e-2                       & 832.34                                    \\
DTMOF                                       & 4.03e-2                 & 3.46e-2                   & 9.15e-2                      & 7.66e-2                       & 1                                         \\ \midrule
Grid: $100 \times 100 \times 50$                                         & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}                             & \multicolumn{1}{l}{}                      \\ \midrule
ELVIRA \citep{pilliod_second-order_2004}                                    & 7.33e-2                 & 9.67e-2                   & 1.66e-1                      & 1.37e-1                          & 97.2                                      \\
Analytic MOF\citep{milcent_moment--fluid_2020}                                & 5.57e-2                 & 5.64e-2                   & 8.38e-2                      & 7.65e-2                          & 6.93                                      \\
Conventional MOF \citep{dyadechko_moment--fluid_2005}                                & 5.58e-2                 & 5.64e-2                   & 8.38e-2                      & 7.65e-2                          & 730.97                                    \\
DTMOF                                        & 5.58e-2                 & 5.77e-2                   & 8.54e-2                      & 7.79e-2                          & 1                                         \\ \bottomrule
\end{tabular}
\end{table}
%</tab:translationerror>

%<*tab:zalesakerror>
\begin{table}[tbhp]
  \centering
  \caption{Geometrical error and run-time ratio in Zalesak's disk rotation test}
  \label{tab:zalesakerror}
\begin{tabular}{@{}llllllll@{}}
\toprule
Method       & $E_g (50)$     & $E_g (100)$    & $E_g (200)$    & $O_h(50)$ & $O_h(100)$ & Run-time ratio       \\ \midrule
ELVIRA \citep{pilliod_second-order_2004}       & 4.26e-03 & 1.89e-03 & 7.90e-04 & 1.17   & 1.25   & 56.7   \\
Analytic MOF \citep{milcent_moment--fluid_2020} & 2.31e-03 & 8.59e-04 & 3.27e-04 & 1.42   & 1.39   & 6.21   \\
Conventional MOF \citep{dyadechko_moment--fluid_2005} & 2.31e-03 & 8.59e-04 & 3.27e-04 & 1.42   & 1.39   & 452    \\
DTMOF        & 2.31e-03 & 8.72e-04 & 3.48e-04 & 1.40   & 1.33   & 1     \\ \bottomrule
\end{tabular}
\end{table}
%</tab:zalesakerror>

%<*tab:reversevortexerror>
\begin{table}[tbhp]
  \centering
  \caption{Geometrical error and run-time ratio in deformation test}
  \label{tab:reversevortexerror}
\begin{tabular}{@{}lllllll@{}}
\toprule
Method       & $E_g (50)$     & $E_g (100)$    & $E_g (200)$    & $O_h(50)$ & $O_h(100)$ & Run-time ratio       \\ \midrule
ELVIRA \citep{pilliod_second-order_2004}      & 5.39e-3 & 1.22e-3  & 3.63-4 & 2.14   & 1.75   & 42.52 \\
Analytic MOF \citet{milcent_moment--fluid_2020} & 3.26e-3 & 9.67e-4 & 1.95e-4 & 1.75   & 2.31   & 8.59  \\
Conventional MOF \citep{dyadechko_moment--fluid_2005} & 3.22e-3 & 9.67e-4 & 1.95e-4 & 1.74   & 2.31   & 577.36 \\
DTMOF        & 3.26e-3 & 1.02e-3 & 1.96e-4 & 1.68   & 2.37   & 1           \\ \bottomrule
\end{tabular}
\end{table}
%</tab:reversevortexerror>
